Neural Part Priors: Learning to Optimize Part-Based Object Completion in RGB-D Scans

3D object recognition has seen significant advances in recent years, showing impressive performance on real-world 3D scan benchmarks, but lacking in object part reasoning, which is fundamental to higher-level scene understanding such as inter-object similarities or object functionality. Thus, we propose to leverage large-scale synthetic datasets of 3D shapes annotated with part information to learn Neural Part Priors (NPPs), optimizable spaces characterizing geometric part priors. Crucially, we can optimize over the learned part priors in order to fit to real-world scanned 3D scenes at test time, enabling robust part decomposition of the real objects in these scenes that also estimates the complete geometry of the object while fitting accurately to the observed real geometry. Moreover, this enables global optimization over geometrically similar detected objects in a scene, which often share strong geometric commonalities, enabling scene-consistent part decompositions. Experiments on the ScanNet dataset demonstrate that NPPs significantly outperforms state of the art in part decomposition and object completion in real-world scenes.

==> Neural Part Priors CVPR 2023/sec/0_abstract.tex <==
\begin{abstract}
3D scene understanding has seen significant advances in recent years, but has largely focused on object understanding in 3D scenes with independent per-object predictions.
%mostly focusing on making predictions as single forward passes, while neglecting to learn the efficiently structured and rich latent spaces. 
We thus propose to learn \OURSFULL{} (\OURS{}), parametric spaces of objects and their parts, that enable optimizing to fit to a new input 3D scan with global scene consistency constraints. 
The rich structure of our \OURS{} enables accurate, holistic scene reconstruction across similar objects in the scene. 
Both objects and their part geometries are characterized by coordinate field MLPs, facilitating optimization at test time to fit to input geometric observations as well as similar objects in the input scan. 
This enables more accurate reconstructions than independent per-object predictions as a single forward pass, while establishing global consistency within a scene.
Experiments on the ScanNet dataset demonstrate that \OURS{} significantly outperforms the state-of-the-art in part decomposition and object completion in real-world scenes.

{\normalfont Project page:} {\normalfont \url{ alexeybokhovkin.github.io/neural-part-priors/}}
\end{abstract}



==> Neural Part Priors CVPR 2023/sec/0_metadata.tex <==

\newcommand{\OURS}{NPPs}
\newcommand{\OURSFULL}{Neural Part Priors}

%\title{[CVPR2022] Official LaTeX Template}
\title{\OURSFULL{}: Learning to Optimize Part-Based Object Completion in RGB-D Scans} %TODO update
% optimized part priors


\author{Andrea Tagliasacchi\\
Google Research \& University of Toronto\\
{\tt\small taglia@google.com}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
% \and
% Second Author\\
% Institution2\\
% First line of institution2 address\\
% {\tt\small secondauthor@i2.org}
}

==> Neural Part Priors CVPR 2023/sec/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}
% 

With the introduction of commodity RGB-D sensors (e.g., Microsoft Kinect, Intel RealSense, etc.), remarkable progress has been made in reconstruction and tracking to construct 3D models of real-world environments \cite{newcombe2011kinectfusion,whelan2015elasticfusion,choi2015robust,niessner2013real,dai2017bundlefusion}.
This has enabled construction of large-scale datasets of real-world 3D scanned environments \cite{dai2017scannet,Matterport3D}, enabling significant advances in 3D semantic segmentation \cite{dai20183dmv,graham20183dsemantic,choy20194d}, 3D semantic instance segmentation \cite{hou20193dsis,engelmann20203d,han2020occuseg}, and even part-level understanding of scenes~\cite{bokhovkin2021towards}.
The achieved 3D object recognition has shown impressive advances, but methods focus on independent predictions per object in single forward passes, resulting in semantic predictions that are inconsistent between repeated objects in a scene, and/or geometric predictions that do not precisely match input observed geometry.

Simultaneously, recent advances in representing 3D shapes as continuous implicit functions represented with coordinate field MLPs have shown high-fidelity shape reconstruction \cite{park2019deepsdf, chibane2020ifnet, chen2019imnet, sitzmann2019siren, chibane2020ndf}.
Such methods have focused on object-level reconstructions, whereas part-based understanding is fundamental to many higher-level scene understanding tasks (e.g., interactions often occur with object parts -- sitting on the seat of a couch, opening a door with a handle, etc.).

%Simultaneously, significant work has been done towards part segmentation on 3D shapes, where synthetic datasets are available with part annotations for supervision \cite{mo2019partnet}. Recently, Bokhovkin et al.~\cite{bokhovkin2021towards} proposed to bridge two tasks together to predict part decompositions of objects in real-world 3D scenes, leveraging part information from synthetic CAD models aligned to real-world scanned scenes \cite{avetisyan2019scan2cad,shapenet2015,dai2017scannet}. This made an important step towards part-based understanding in 3D scenes. However, due to a single forward pass prediction, the aforementioned methods and Bokhovkin et al. focus on independent per-object prediction and are not able to reconstruct every shape in a dataset with acceptable accuracy on average, but not in particular, as optimization-based methods do. These approaches are not able to keep enough accuracy between predicted geometry and the actual underlying scan geometry and a sufficient level of consistency between predicted shapes belonging to one scene. Nevertheless, the greatest drawbacks of the latter are long runtime and the requirement of proper initialization. In addition, Bokhovkin et al.~\cite{bokhovkin2021towards} treats each object on a scene independently and is not able to achieve high accuracy surface reconstruction due to a dense volumetric representation, relying heavily on synthetic priors that did not match precisely to real observations.

We thus propose to learn \OURSFULL{} (\OURS{}), optimizable parametric shape and part spaces learned from synthetic data.
These learned manifolds enable efficient traversal in latent spaces during inference to fit precisely to objects in real-world scanned scenes, while maintaining consistent part decompositions with similar objects in the scene. 
Our \OURS{} leverage the representation power of neural implicit functions encoded as coordinate-field MLPs, representing both shape and part geometries of objects.
A shape can then be represented by a set of latent codes for each of its parts, where each code decodes to predict the respective part segmentation and signed distance field representation of the part geometry.
This representation enables effective \textit{test-time joint optimization} over all parts of a shape by traversing through the part latent space to find the set of parts that best explain a real-world shape observation.
Furthermore, as repeated objects often appear in a scene under different partial observation patterns (resulting in inconsistent predictions when made independently for each object) we further optimize for part consistency between similar objects detected in a scene to produce scene-consistent part decompositions. This allows us to reconstruct the holistic structure of a scene. 

To fit real-world 3D scan data, we first perform object detection and estimate the part types for each detected object.
We can then optimize \textit{in test time} jointly over the part codes for each shape to fit the observed scan geometry; we leverage a predicted part segmentation of the detected object and optimize jointly across the parts of each shape such that each part matches the segmentation, and their union fits the object.
This joint optimization across parts produces a high-resolution part decomposition whose union represents the complete shape while fitting precisely to the observed real geometry.
Furthermore, this optimization at inference time allows leveraging global scene information to inform our optimized part decompositions; in particular, we consider objects of the same predicted class with similar estimated geometry, and optimize them jointly, enabling more robust and scene-consistent part decompositions.

%TODO HERE

In summary, we present the following contributions:
\begin{itemize}[leftmargin=*]
\setlength\itemsep{-.3em}
\item We propose to learn optimizable part-based latent priors for 3D shapes -- \OURSFULL{}, encoding part segmentation and part geometry into a latent space for the part types of each class category.

\item Our learned, optimizable part priors enable test-time optimization over the latent spaces, enhanced with \textit{inter-shape part-based constraints}, to fit partial, cluttered object geometry in real-world scanned scenes, resulting in robust and precise semantic part completion.

\item We additionally propose a scene-consistent optimization, enhanced with \textit{intra-shape constraints}, jointly optimizing over similar objects that provides globally-consistent part decompositions for repeated object instances in a scene.
\end{itemize}

==> Neural Part Priors CVPR 2023/sec/2_related.tex <==
\vspace{-0.3cm}
\section{Related Works}
\label{sec:related}
\vspace{-0.3cm}

\paragraph{3D Object Detection and Instance Segmentation}
3D semantic scene understanding has seen rapid progress in recent years, with large-scale 3D datasets \cite{dai2017scannet,Matterport3D,geiger2012we} and developments in 3D deep learning showing significant advances in object-level understanding of 3D scenes.
Various methods explore learning on different 3D representations for object detection and instance segmentation, including volumetric grids \cite{hou20193dsis,tung2019learning}, point clouds \cite{qi2019deep,xie2020mlcvnet,jiang2020pointgroup,qi2020imvotenet,nie2021rfd}, sparse voxel representations \cite{engelmann20203d,han2020occuseg}, and hybrid approaches \cite{hou20193dsis,qi2020imvotenet}.
These approaches have achieved impressive performance in detecting and segmenting objects in real-world observations of 3D scenes, but do not consider lower-level object part information that is requisite for many vision and robotics tasks, that involve object interaction and manipulation.

Recently, Bokhovkin et al.~\cite{bokhovkin2021towards} proposed an approach to estimate part decompositions of objects in RGB-D scans, leveraging structural part type prediction and a pre-computed set of geometric part priors.
Due to the use of dense volumetric part priors, the part reasoning is limited to coarse resolutions, and does not precisely match the input observed geometry.
We also address the task of semantic part prediction and completion for objects in real-world 3D scans, but leverage a learned, structured latent space representing neural part priors, enabling part reasoning at high resolutions which optimizing to fit accurately to the observed scan geometry.


\paragraph{3D Scan Completion}
As real-world 3D reconstructions are very often incomplete due to the complexity of the scene geometry and occlusions, various approaches have been developed to predict complete shape or scene geometry from partial observations.
Earlier works focused on voxel-based scan completion for shapes \cite{wu20153d,dai2017shape}, with more recent works tackling the challenge of generating complete geometry from partial observations of large-scale scenes \cite{song2017semantic,dai2018scancomplete,dai2020sgnn,dai2021spsg}, but without considering individual object instances.
Several recent works propose to detect objects in an RGB-D scan and estimate the complete object geometries, leveraging voxel \cite{hou2020revealnet,bokhovkin2021towards} or point \cite{yi2019gspn,nie2021rfd} representations.
Our approach to predicting part decompositions of objects inherently provides object completion as the predicted parts union; in contrast to previous approaches estimating object completion in RGB-D scans, we propose to characterize object parts as learned implicit priors, enabling test-time traversal of the latent space to fit accurately to observed input scan geometry.

\paragraph{Part Segmentation of 3D Shapes}
Part segmentation for 3D shapes has been well-studied in shape analysis, typically focusing on understanding collections of synthetic shapes.
Various methods have been developed for unsupervised part segmentation by finding a consistent segmentation across a set of shapes \cite{golovinskiy2009consistent,huang2011joint,sidi2011unsupervised,hu2012co,luo2020learning}.
Recent deep learning based approaches have leveraged datasets of shapes with part annotations to learn part segmentation on new shapes \cite{kalogerakis20173d,yi2016scalable,hanocka2019meshcnn}.
In particular, approaches that learn part sequences and hierarchies to capture part structures have shown effective part segmentation for shapes \cite{wang2011symmetry,van2013co,yi2017learning,mo2019partnet,mo2019structurenet,wu2020pq}.
These approaches target single-object scenarios, whereas we construct a set of learned part priors that can be optimized to fit to real-world, noisy, incomplete scan geometry.

\paragraph{Neural Implicit Representations of 3D Shapes}
Recently, we have seen significant advances in generative shape modeling with learned neural implicit representations that can represent continuous implicit surface representations, without ties to an explicit grid structure.
Notably, DeepSDF~\cite{park2019deepsdf} proposed an MLP-based network that predicts the SDF value for a given 3D location in space, conditioned on a latent shape code, which demonstrated effective modeling of 3D shapes while traversing the learned shape space.
Such implicit representations have also been leveraged in hybrid approaches coupling explicit geometric locations with local implicit descriptions of geometry for shapes \cite{genova2019learning,genova2020local} as well as scenes \cite{peng2020convolutional}, without semantic meaning to the local decompositions. 
We propose to leverage the representation power of such learned continuous implicit surfaces to characterize semantic object parts that can be jointly optimized together to fit all parts of an object to a partial scan observation.


==> Neural Part Priors CVPR 2023/sec/3_method.tex <==


\section{Method}

% Overview
\begin{figure*}
\begin{center}
    \centering
    \includegraphics[width=0.85\textwidth]{fig/full_overview.jpg}
    \vspace{-0.3cm}
    \caption{Method overview.
    From an input scan, we first detect 3D bounding boxes for objects. 
    For each object, we predict their semantic part structure as a set of part labels and latent codes for each part. 
    These latent codes map into the space of neural part priors, along with a full shape code used to regularize the shape structure.
    We  then refine these codes at test time by optimizing to fit to the observed input geometry along with inter-object consistency between similar detected objects, producing effective part decompositions reflecting complete objects with scene consistency.
    \vspace{-0.9cm}
    }
    \label{fig:overview}
\end{center}%
\end{figure*}

% % Overview
% \begin{figure}
% \begin{center}
%     \centering
%     \includegraphics[width=1.0\textwidth]{fig/overview_1.jpg}
%     \caption{ \TODO{caption}
%     }
%     \label{fig:overview_1}
% \end{center}%
% \end{figure}

% % Overview
% \begin{figure}
% \begin{center}
%     \centering
%     \includegraphics[width=1.0\textwidth]{fig/overview_2.jpg}
%     \caption{ \TODO{caption}
%     }
%     \label{fig:overview_2}
% \end{center}%
% \end{figure}

\subsection{Overview}

We introduce \OURSFULL{} (\OURS{}) to represent learned spaces of geometric object part priors, that enable joint part segmentation and completion of objects in real-world, incomplete RGB-D scans.
From an input 3D scan $\mathcal{S}$, we first detect objects $\mathcal{O}$ = \{$o_i$\} in the scan characterized by their bounding boxes and orientations, then for each object, we predict its part decomposition into a part class categories (with corresponding part latent codes) and their corresponding complete geometry represented as signed distance fields (SDFs) and trained on part annotations for shapes.
This enables holistic reasoning about each object in the scene and prediction of complete geometry in unobserved scan regions.
Since captured real-world scene geometry contains significant incompleteness or noise, we  model our geometric part priors based on complete, clean synthetic object parts, represented as a learned latent space over implicit part geometry functions.
This enables test-time optimization over the latent space of parts to fit real geometry observations, enabling part-based object completion while precisely representing real object geometry.
Rather than considering each object independently, we observe that repeated objects often occur in scenes under different partial observations, leading to inconsistent independent predictions; we thus jointly optimize across similar objects in a scene, where objects are considered similar if they share the same class category and predicted shape geometries are close by chamfer distance. This results in scene-consistent, high-fidelity characterizations of both object part semantics and complete object geometry.
%\ALEX{During test-time optimization (TTO) we also incorporate two types of consistency constraints. First, we force optimization of parts geometry in TTO to be guided with an optimization of full shape geometry. This helps to keep completeness of every optimized part and consistency between parts. Second, we make use of similar instances on a scene with our scene-aware consistency constraints. We identify similar objects on a scan that have the same shape category and aggregate information from all of them to produce a unified shape.}
An overview of our approach is shown in Fig.~\ref{fig:overview}. 

% Our \OURS{} spaces characterize object part geometry as signed distance fields (SDFs), trained on part annotations for shapes.
% For each detected object $o_i\in \mathcal{O}$ in an input scan, we predict its semantic parts as the set of part categories that compose the object along with initial estimates of their corresponding latent codes in the learned part space.
% We then optimize for refined object pose alignment, and then for the part latent codes to fit to the observed geometry of each $o_i$.
% For objects of the same class category and with similar predicted shape geometry by chamfer distance, we jointly constrain them together in this optimization.
% This results in scene-consistent, high-fidelity characterizations of both object part semantics and complete object geometry.


\subsection{Object Detection}
From input 3D scan $\mathcal{S}$, we first detect objects in the scene, leveraging a state-of-the-art 3D object detection backbone from MLCVNet~\cite{xie2020mlcvnet}.
MLCVNet interprets $\mathcal{S}$ as a point cloud and proposes objects through voting~\cite{qi2019deep} at multiple resolutions, providing an output set of axis-aligned bounding boxes for each detected object $o_i$.
We extract the truncated signed distance field $D_i$ for each $o_i$ at $4$mm resolution to use for test-time optimization.
We then aim to characterize shape properties for $o_i$ to be used for rotation estimation and test-time optimization, and interpret $D_i$ as a $32^3$ occupancy grid which is input to a 3D convolutional object encoder to produce the object's shape descriptor $\mathbf{s}_i\in\mathbb{R}^{256}$.
%\ANGIE{we extract both 32 occupancy and high-res sdf? the occupancy for the model and the sdf for test time fitting instead of sdf as input to the model?} \ALEX{Yes, we extract first high-res sdf with resolution of 4 mm, then convert this field to occupancy by threshold $abs(sdf) < 0.02$}

\paragraph{Initial Rotation Estimation} From $\mathbf{s}_i$, we use a 2-layer MLP to additionally predict an initial rotation estimate of the object as $r_i^{\mathrm{init}}$ around the up (gravity) vector of $\mathcal{S}$.
We note that the up vectors of an RGB-D scan can be reliably estimated with IMU and/or floor estimation techniques \cite{dai2017scannet}.
The rotation estimation is treated as a classification problem across $n_{r}=12$ bins of discretized angles ($\{0^{\circ}, 30^{\circ}, \dots, 330^{\circ}\}$), using a cross entropy loss.
We use the estimated rotation $r_i^{\mathrm{init}}$ to resample $D_i$ to approximate the canonical object orientation, from which we use to optimize for the final rotation $r_i$ and the object part latent codes.


%We then resample the input scan geometry within each detected box into $32^3$ occupancy grids $o_i\in \mathbb{O}$ to inform our part decomposition. In addition, we extract a truncated signed distance field (tSDF) $sdf_i$ within predicted bounding box, where truncation distance is $0000$ and tSDF resolution is $0000$ cm. Truncated SDFs are obtained with fusion of depthmaps.
%For a detected object $o_i$ from the scan, represented as a $32^3$ occupancy grid of the scan geometry within its predicted bounding box, we encode the occupancy grid with  four 3D convolutional blocks (consisting of convolution, group normalization and ReLU activation) and extract a feature encoding $z_i$ of dimension $256$, which is used to inform the part decomposition. 

%\paragraph{Object Orientation Prediction}
%Since our object detection backbone predicts axis-aligned bounding boxes for each object, we additionally predict the orientation $r_i$ of each object $o_i$ from its feature $z_i$ using an MLP.
%We assume that the up (gravity) vector is known in the scene, and thus predict the angle around the up vector by classifying the angle in $n_{\alpha}=12$ bins of discretized angles ($\{0^{\circ}, 30^{\circ}, \dots, 330^{\circ}\}$) with a cross entropy loss.
%The predicted object orientation allows us to initialize the orientation of input signed distance field $sdf_i$ for the following ICP registration, decribed in Section~\ref{}.


\subsection{Learned Space of \OURSFULL{}}
We first learn a set of latent part spaces for each class category, where each part space represents all part types for the particular object category.
To this end, we employ a function $f_p$ characterized as an MLP to predict the implicit signed distance representation for each part geometry of the class category.
In addition to the latent part space, we additionally train a proxy shape function $f_s$ as an MLP that learns full shape geometry as implicit signed distances, which will serve as additional regularization during the part optimization.
Both $f_p$ and $f_s$ are trained in auto-decoder fashion following DeepSDF~\cite{park2019deepsdf}.
Then each train shape part is embedded into a part latent space by optimizing for its code  $\mathbf{z}^{\mathrm{p}}_k\in \mathbb{R}^{256}$ such that $f_p$ conditioned on this code and the part type maps a positional encoding $\mathbf{x}^{pos}\in\mathbb{R}^{63}$ of a point $\mathbf{x}\in\mathbb{R}^3$ in the canonical space to SDF value $d$ of the part geometry:
\begin{equation}
    f_p: \mathbb{R}^{63} \times \mathbb{R}^{256}\times \mathbb{Z}_2^{N_c} \rightarrow\mathbb{R}, \quad\quad f_p(\mathbf{x}^{pos},\mathbf{z}^{\mathrm{p}}_k,\mathds{1}_{\mathrm{part}})=d.
\end{equation} 
where $\mathds{1}_{\mathrm{part}}\in\mathbb{Z}_2^{N_c}$ is a one-hot encoding of the part type for a maximum of $N_c$ parts. Similar to NeRF~\cite{mildenhall2020nerf}, euclidean coordinates $\mathbf{x}\in\mathbb{R}^3$ are encoded using $\sin/\cos$ functions with 10 frequencies $[2^0,...,2^9]$.
The shape space is trained analogously for each class category where $\mathbf{z}^{\mathrm{s}}_i\in \mathbb{R}^{256}$ represents a shape latent code in the space:
%Similarly, each shape is encoded into a latent code $\mathbf{z}^{\mathrm{s}}_i\in \mathbb{R}^{256}$ \ALEX{Similarly, each shape is embedded into a DeepSDF shape latent space as a code $\mathbf{z}^{\mathrm{s}}_i\in \mathbb{R}^{256}$}, with the $f_s$ mapping a point $\mathbf{x}\in\mathbb{R}^3$ in the canonical space to an SDF value $d$, conditioned on $z^{\mathrm{s}}_i$:
\begin{equation}
    f_s: \mathbb{R}^{63} \times \mathbb{R}^{256}\rightarrow\mathbb{R}, \quad\quad f_p(\mathbf{x}^{pos},\mathbf{z}^{\mathrm{s}}_i)=d.
\end{equation}
%We try our method for several furniture categories, such as chairs, tables, beds etc. To perform efficient inference that includes optimization in test-time in implicit domain we need powerful and implicit priors for shape and part category. The DeepSDF approach is able to provide such priors, where they are represented as combinations of learned DeepSDF latent space and MLP (multi-layer perceptron) decoder. Thus, for every shape category we train $2$ types of decoders. One is trained for the whole shapes: $$s = MLP_{shape}([x, lat]),\ x \in \mathbb{R}^3,\ lat\in \mathbb{R}^{256},\ s \in \mathbb{R},$$ another one is trained for all parts of all shapes: $$s = MLP_{part}([x, lat, \mathds{1}_{part}]),\ x \in \mathbb{R}^3,\ lat\in \mathbb{R}^{256},\ s \in \mathbb{R},$$ where $x$ is a 3D point, $s$ is a corresponding distance to a surface, $lat$ is a shape or part latent vector, $\mathds{1}_{part} \in \mathbb{R}^{n^{part}_c}$ is a one-hot vector of a part type ($n^{part}_c$ -- number of parts for an arbitrary shape category $c$). 
%To pretrain these MLPs as implicit functions we follow the original DeepSDF approach, where we use ShapeNet~\cite{} dataset of synthetic shapes and split every shape on parts using PartNet~\cite{} labels. 

We train latent spaces of part and shape priors on the synthetic PartNet~\cite{mo2019partnet} dataset to characterize a space of complete parts and shapes, by minimizing the reconstruction error over all train shape parts, while optimizing for latent codes $\{ \mathbf{z}^{\mathrm{p}}_k \}$ and weights of $f_p$.
We use an $\ell_1$ reconstruction loss with $\ell_2$ regularization on the latent codes:
\begin{equation}
    L = \sum_{j=1}^{N_p} |f_p(\mathbf{x}_j^{pos},\mathbf{z}^{\mathrm{p}}_k,\mathds{1}_{\mathrm{part}}) - D^\textrm{gt}(\mathbf{x}_j^{pos})|_1 + \lambda||\mathbf{z}^{\mathrm{p}}_k||_2^2
\end{equation}
for $N_p$ points near the surface, the regularization weight $\lambda=$1e-5.
We train $f_s$ analogously.

\begin{figure*}
\centering
\begin{subfigure}{.52\textwidth}
  \centering
    \includegraphics[width=1.0\textwidth]{fig/overview_1.jpg}
    \caption{ Projection into part and shape spaces.
    }
    \label{fig:overview_1}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
    \includegraphics[width=1.0\textwidth]{fig/overview_2.jpg}
    \caption{ Joint optimization to fit to input scan.
    }
    \label{fig:overview_2}
\end{subfigure}
\vspace{-0.2cm}
\caption{(a) Projection into the part and shape latent spaces along with part segmentation from input scan geometry. (b) Optimization at test time to fit to observed scan geometry while maintaining inter-part consistency within a shape and inter-shape consistency for geometrically similar objects.}
\vspace{-0.2cm}
\label{fig:test}
\end{figure*}


\subsection{Part Decompositions in Real Scenes}

Once we have learned our latent space of parts, we can traverse them at test time to find the part-based decomposition of an object that best fits to its real-world observed geometry in a scene.
Since real-world observations are typically incomplete, we can optimize for complete part decompositions based on strong priors given by the trained latent spaces.
This allows for effective regularization by synthetic part characteristics (clean, complete) while fitting precisely to real observed geometry.

To guide this optimization for a detected object box $o$ with its shape feature $\mathbf{s}$, we predict its high-level decomposition into a set of semantic part types $\{(c_k, \mathbf{p}_k)\}$, where $\mathbf{p}_k\in\mathbb{R}^{256}$ is a part feature descriptor and $c_k$ the part class label.
The $i$ object suffix is discarded here for simplicity.
The part optimization is initialized using $\{(c_k, \mathbf{p}_k)\}$.

To obtain the semantic part type predictions, we employ a message-passing graph neural network that infers part relations to predict the set of component part types.
Similar to \cite{mo2019structurenet}, from the shape feature $\mathbf{s}$ we use an MLP to predict at most $N_c=10$ parts.
For each potential part $k$, we predict its probability of existence, its part label $c_k$, its feature vector $\mathbf{p}_k$, and probabilities of physical adjacency (given by face connectivity between parts) between each pair of parts to learn structural part information.
This produces the semantic description of the set of parts for the object $\{(c_k, \mathbf{p}_k)\}$, from the parts predicted with part existence probability $>0.5$.

\paragraph{Projection to the Latent Part Space}
We then learn a projection mapping from the part features $\{\mathbf{p}_k\}$ to the learned latent part space based on synthetic part priors, using a small MLP to predict $\{\tilde{\mathbf{z}}_k^\textrm{p}\}$, as shown in Fig.~\ref{fig:test}(a).
This helps to provide a close initial estimate in the latent part space in order to initialize optimization over these part codes to fit precisely to the observed object geometry.
Similarly, we project the shape code $\mathbf{s}$ to the learned latent shape space with a small shape projection MLP to predict $\{\tilde{\mathbf{z}}^\textrm{s}\}$, which we use to help regularize the part code optimization.
Both of these projection MLPs are trained using MSE losses against the optimized train codes of the latent spaces.
%Both of these projection MLPs consist of 4 $512$ neuron layers with ReLU activations, and are trained using MSE losses against the optimized train codes of the latent spaces.

\paragraph{Part Segmentation Estimation}\label{subsec:pointcls}
In addition to our projection initialization, we estimate part segmentation $\{D^{\textrm{p}}\}_{\textrm{p}=1}^{N_{parts}}$ for the input object TSDF $D$ over the full volume, representing part SDF geometry in the regions predicted as corresponding to the part p, where part segmentation regions cover the entire shape, including unobserved regions.
This is used to guide part geometry predictions when optimizing at test time to fit to real observed input geometry. 
For each point $\mathbf{x}\in\mathbb{R}^3$ which has distance $<d_{trunc} = 0.16$m from the input object TSDF $D$, we classify it to one of the predicted parts $\{(c_k, \mathbf{p}_k)\}$ or background using a small PointNet-based\cite{qi2017pointnet} network.
This segmentation prediction takes as input the corresponding shape feature $\mathbf{s}$, the initial estimated rotation $r_i^{\mathrm{init}}$, and the 3D coordinates of $\mathbf{x}$, and is trained with a cross-entropy loss.

% In addition to our projection initialization, we estimate part segmentation for the input object TSDF $D$ over the full volume, representing complete part segmentation; this is used to guide part geometry predictions to avoid self-intersections between part geometries.
% We thus predict whether a given point $\mathbf{x}\in\mathbb{R}^3$ should be associated with a part code $\mathbf{z}_k^\textrm{p}$ which decodes to an implicit SDF function $d_k$.
% We formulate this association through contrastive learning: point locations associated with their ground truth part geometry $(\mathbf{x}, \mathbf{z}_k^\textrm{p}, d_k)\in\mathbb{R}^{260}$ are considered to all be positive, while non-corresponding point-parts  $(\mathbf{x}, \mathbf{z}_j^\textrm{p}, d_k)\in\mathbb{R}^{260}, j\neq k$ are negative.
% We use a small MLP with a sigmoid activation to predict $1$ for positive vectors and $0$ for negatives.
% Note that this formulation allows part segmentation to be agnostic to the number of parts.
% Additionally, points not associated with any part (those with sigmoid activation $<0.5$) are considered as background, and ignored during part optimization.

%As we want to reconstruct each part in implicit domain, we need to provide local non-intersecting signed distance fields for all parts. It is important to classify points of the input field $sdf_i$ with high accuracy to avoid predicting self-intersecting parts in test time. We perform point classification in a contrastive manner. Taking an arbitrary point $x_{p_k} \in \mathbb{R}^3$ with a corresponding signed distance $s_{p_k} \in \mathbb{R}$ (where $p_k$ denotes a particular part, $k \in \{1, \dots, n^{part}\}$, $n^{part}$ -- number of existing latent vectors $z'_k$) and all existing latent vectors $z'_k$ we form positive $[x_{p_k}, s_{p_k}, z'_k] \in \mathbb{R}^{260}$ and negative $[x_{p_k}, s_{p_k}, z'_j] \in \mathbb{R}^{260}\ (j\neq k)$ vectors. These vectors are taken as input to a small MLP with a sigmoid activation, which is trained to predict $1$ for positive vectors and $0$ for negatives. This approach allows our classification network to be agnostic of number of different parts for a shape category $c$. At the same time we can separate points that belong to background by filtering all the predicted sigmoid activations with a threshold less than $\theta_{bck}=0.5$.

\subsection{Joint Inter- and Intra-Shape Part Optimization}\label{subsec:partopt}
To obtain the final part decompositions, we traverse over the learned latent part space to fit to the observed input scan geometry, as shown in Fig.~\ref{fig:test}(b).
From the initial estimated part codes $\{\tilde{\mathbf{z}}_k^\textrm{p}\}$ and shape code $\{\tilde{\mathbf{z}}^\textrm{s}\}$, their decoded part SDFs should match to each of $\{D^{\textrm{p}}\}_{\textrm{p}=1}^{N_{parts}}$.
%
Since the part and shape latent spaces have been trained in the canonical shape space, we optimize for a refined rotation prediction $r$ from $r^\textrm{init}$ using iterative closest points \cite{besl1992method,rusinkiewicz2001efficient} between the sampled points near $D$ and the initial shape estimate from projection $\tilde{\mathbf{z}}^\textrm{s}$.
We use $N_i$ sampled points near the observed input surface $D$ (near being SDF values $<0.025$m) for rotation refinement, with $N$ the number of points not predicted as background during part segmentation.
%\ALEX{We also denote $N$ as number of points not being predicted as background from $D$.}

%We then predict the final part decomposition in two stages. First, for each element $\{z'_k\}$ in the predicted semantic part arrangement $T_i$, we perform inference with DeepSDF decoders to obtain initial complete signed distance fields $\overline{sdf}^{shape}_i$ for the whole shape and $\{\overline{sdf}^{part}_1,\dots,\overline{sdf}^{part}_{n^{part}}\}$ for corresponding parts. After that we can subsample predicted fields to near-surface points $sdf'^{shape}_i$ and $\{\overline{sdf}'^{part}_1,\dots,\overline{sdf}'^{part}_{n^{part}}\}$ by taking only the points with distance less than threshold $\theta_{surf}=0.005$. The same operation is performed for the input field $sdf_i$ of a scan to get a $sdf'_i$.
%To enable efficient and accurate overfitting to a particular example in test time we perform preliminary ICP registration of the predicted $\overline{sdf}'^{shape}_i$ with the $sdf'_i$ from a scan to get a registration transformation $M$. After that we classify the points of partial field $sdf_i$ to parts $\{sdf^{part}_1,\dots,sdf^{part}_{n^{part}}\}$ using an approach of Section~\ref{subsec:pointcls} and apply transform $M$ to get $sdf'_i$ and $\{sdf'^{part}_1,\dots,sdf'^{part}_{n^{part}}\}$.

%\paragraph{Part-based Implicit Test-Time Optimization}
While the predicted projected part and shape codes $\{\tilde{\mathbf{z}}_k^\textrm{p}\},\{\tilde{\mathbf{z}}_k^\textrm{s}\}$ can provide a good initial estimate of the part decomposition of the complete shape, they represent synthetic part and shape priors that often do not fit the observed real input geometry.
We thus optimize for part decompositions that best fit the input observations by minimizing the energy:
\begin{equation}\label{eq:optimization}
    L = \sum_k L_{\textrm{part}} + L_{\textrm{shape}} + w_\textrm{cons} L_{\textrm{cons}},
\end{equation}
where $L_{\textrm{part}}$ denotes the part reconstruction loss, $L_{\textrm{shape}}$ a proxy shape reconstruction loss, $L_{\textrm{cons}}$ a regularization to encourage global part consistency within the estimated shape, and $w_\textrm{cons}$ is a consistency weight.

$L_{\textrm{part}}$ is an $\ell_1$ loss on part reconstruction:
\begin{equation}\label{eq:parts}
    L_{\textrm{part}} = \sum_{\textrm{p}=1}^{N_{parts}}\sum_{N^{\textrm{p}}} w_{trunc}|f_p(\mathbf{z}_k^\textrm{p}) - T_r(D^\textrm{p})| + \lambda||\mathbf{z}^{\mathrm{p}}_k||_2^2,
\end{equation}
where $N^{\textrm{p}}$ is the number of points classified to part $\textrm{p}$ and  $w_{trunc}$ gives a fixed greater weight for near-surface points ($<d_{trunc} = 0.16$m). % than those further away.
%\ALEX{and $w_{trunc}$ switches between points near the surface (less than $d_{trunc} = 0.16$m) than those further away}. 

$L_{\textrm{shape}}$ is a proxy $\ell_1$ loss on shape reconstruction:
\begin{equation}\label{eq:shape}
    L_{\textrm{shape}} = \sum_{N} w_{trunc}|f_s(\mathbf{z}^\textrm{s}) - T_r(D)| + \lambda||\mathbf{z}^{\textrm{s}}||_2^2.
\end{equation}

The regularization weight $\lambda=$1e-5 for both Eq.~\ref{eq:parts},~\ref{eq:shape}. Finally, $L_{\textrm{cons}}$ encourages all parts to reconstruct a shape similar to the optimized shape:
\begin{equation}\label{eq:cons}
    L_{\textrm{cons}} = \sum_{N} |f_p(\mathbf{z}_k^\textrm{p}) - f_s(\mathbf{z}^\textrm{s})|,
\end{equation}
where $f_s(\mathbf{z}^\textrm{s})$ is frozen for $L_{\textrm{cons}}$.
This allows for reconstructed parts to join together smoothly without boundary artifacts to holistically reconstruct a shape.

This produces a final optimized set of parts for each object in the scene, where parts both fit precisely to input geometry and represent the complete geometry of each part, even in unobserved regions.
The final part geometries can be extracted from the SDFs with Marching Cubes~\cite{lorensen1987marching} to obtain a surface mesh representation of the semantic part completion.

\paragraph{Scene-Consistent Optimization}
% While this formulation enables joint part optimization within an object, we observe that multiple objects within a scene often tend to correlate with each other.
Scenes often contain repeated instances of objects which are observed from different views, thus frequently resulting in inconsistent part decompositions when considered as independent objects.
We propose a scene-consistent optimization between similar predicted objects, where objects in a scene are considered similar if their predicted class category is the same and the chamfer distance between their decoded shapes from $\tilde{\mathbf{z}}_k^\textrm{s}$ is $<\tau_s$.

For a set of $N_{sim}$ similar objects in a scene, we collect together their predicted part segmentations and observed input SDF geometry in the canonical orientation based on $T_r(D^\textrm{p})$ to provide a holistic set of constraints across different partial observations to produce $\{D_i\}_{i = 1}^{N_{sim}}$. 
The $\{D_i\}_{i = 1}^{N_{sim}}$ are then aggregated to form $\mathbf{D'}$ by sampling a set of $N_{avg}$ points near the surfaces of $\{D_i\}_{i = 1}^{N_{sim}}$ where $N_{avg}$ is the average number of points across the $N_{sim}$ objects, and each point is assigned the minimum SDF value within its 30-point local neighbourhood (to help ensure that objects do not grow thicker in size from small-scale misalignments).
Based on  $\mathbf{D'}$, we then optimize for the part decompositions following Eq.~\ref{eq:optimization}.
%


%So far as we have already predicted 3D priors for a shape ($\overline{sdf}^{shape}_i$) and corresponding parts ($\{\overline{sdf}'^{part}_1,\dots,\overline{sdf}'^{part}_{n^{part}}\}$), estimated ICP alignment $M$ of input scan tSDF $sdf_i$ and classified the points of it, we are able to perform even tighter fitting of local partial parts fields $\{sdf'^{part}_1,\dots,sdf'^{part}_{n^{part}}\}$. For this aim we propose the algorithm~\ref{subsec:ttoalgo}. As DeepSDF models can work only as a combination of a learned latent space and a corresponding MLP decoder, it is clear that tuning decoder weights at great extent can disturb priors and destroy complete and consistent geometry of parts. To avoid this we propose several constraints during test-time optimization. According to our algorithm we optimize our part decoders in partwise manner. As distance fields of real-world scans are commonly incomplete we use predictions of $MLP_{shape}$ as a guidance for $MLP_{part}$ optimization. Namely, we constraint predictions of $MLP_{part}$ for every part to be close to predictions of $MLP_{shape}$, because this MLP is not able to go beyond its latent space, in contrast to $MLP_{part}$ which can also optimize its weights. 


\begin{comment}
\begin{algorithm}\label{subsec:ttoalgo}
\DontPrintSemicolon
  
  \KwInput{Predicted shape and parts projections $e'_{shape}$ and $\{e'_1,\dots,e'_{n^{part}}\}$, shape MLP decoder $MLP_{shape}$, part MLP decoder $MLP_{part}$, number of iterations $num\_iterations$, consistency weight $w_{cons}$}
  \KwOutput{Optimized shape and parts projections $\overline{e'_i}$ and $\{\overline{e'_1},\dots,\overline{e'_{n^{part}}}\}$, optimized shape and part MLP decoders $\overline{MLP_{shape}}$ and $\overline{MLP_{part}}$, final meshes of parts $\{Mesh_1,\dots,Mesh_{n^{part}}\}$}
  \KwData{Aligned partial tSDFs for parts $SDF_{part}=\{sdf'^{part}_1,\dots,sdf'^{part}_{n^{part}}\}$, aligned partial tSDF for shape $sdf'$}
  
  $w_{part}^{init} = \text{weights}(MLP_{part})$
  
  \For{$sdf'^{part}_k$ \textbf{in} $SDF_{part}$}{
  $\text{weights}(MLP_{part}) = w_{part}^{init}$
  
  Set trainable $e'_k$, $e'_{shape}$
  
  $coord^{part}_k,\ dist^{part}_k = sdf'^{part}_k$
  
  $coord^{shape},\ dist^{shape} = sdf'$
  
    \For{$i=0$ \textbf{to} $i < num\_iterations$}{
    
        \If{$i > 200$}{
        Set trainable $\text{weights}(MLP_{part})$
        }
    
    $\overline{dist^{part}_k} = MLP_{part}(coord^{part}_k)$
    
    $\overline{dist^{shape}} = MLP_{shape}(coord^{shape})$
    
    $\overline{\overline{dist^{part}_k}} = MLP_{shape}(coord^{part}_k)$
    
    $L_{part} = L_1(\overline{dist^{part}_k}, dist^{part}_k)$
    
    $L_{shape} = L_1(\overline{dist^{shape}}, dist^{shape})$
    
    $L_{cons} = L_1(\overline{dist^{part}_k}, \overline{\overline{dist^{part}_k}})$
    
    $L = L_{part} + L_{shape} + w_{cons}\cdot L_{cons}$
    
    $L.backward()$
    
    Optimization step
    }
    $\overline{e'_k} = e'_k$
    
    $\overline{w_{part}} = \text{weights}(MLP_{part})$
    
    $SDF_k = MLP_{part}[\overline{e'_k},\ \overline{w_{part}}](\mathbb{R}^3)$
    
    $Mesh_k = MarchingCubes(SDF_k)$
  }

\caption{Shape and Parts Test-Time Optimization}
\end{algorithm}
\end{comment}


\subsection{Implementation Details}
We first train our latent part and shape spaces on per-category on the synthetic PartNet~\cite{mo2019partnet} dataset.
We then train the projection mapping into the learned part and shape spaces as well as the part segmentation.
This is first pre-trained on synthetic PartNet data using virtually scanned incomplete inputs to take advantage of the large amount of synthetic data.
To apply to real-world observations, we then fine-tune the projections and part segmentation on ScanNet~\cite{dai2017scannet} data using MLCVNet~\cite{xie2020mlcvnet} detections on train scenes. 

In test time, we optimize for part and shape codes using an Adam optimizer with learning rate of 3e-4 for 300 iterations and 3e-5 for the next 300 iterations.
To enable more flexibility to capture input details, we optimize the decoder weights for parts and shape after 400 iterations. 
Optimization for each part takes $\approx 25$ seconds.
For further implementation and training details, we refer to the supplemental.

==> Neural Part Priors CVPR 2023/sec/4_results.tex <==
\begin{table*}[tp]
\centering
\resizebox{\textwidth}{!}{
\vspace{-0.5cm}
\begin{tabular}{l|cccccc|cc||cccccc|cc}
& \multicolumn{8}{c||}{Chamfer Distance -- Accuracy ($\downarrow$)} & \multicolumn{8}{c}{Chamfer Distance -- Completion ($\downarrow$)}\\
\toprule
    Method & chair & table & cab. & bkshlf & bed & bin & class avg & inst avg & chair & table & cab. & bkshlf & bed & bin & class avg & inst avg \\
\midrule
    SG-NN\cite{dai2020sgnn} + MLCVNet\cite{xie2020mlcvnet} + PointGroup\cite{jiang2020pointgroup} & 0.047 & 0.110 & 0.146 & 0.173 & 0.350 & 0.051 & 0.146 & 0.083 & 0.054 & 0.141 & 0.123 & 0.192 & 0.382 & 0.045 & 0.156 & 0.089 \\
    MLCVNet\cite{xie2020mlcvnet} + StructureNet\cite{mo2019structurenet} & 0.024 & 0.074 & 0.104 & 0.166 & 0.424 & 0.039 & 0.138 & 0.061 & 0.028 & 0.129 & 0.118 & 0.154 & 0.352 & 0.037 & 0.136 & 0.067 \\
    Bokhovkin et al.\cite{bokhovkin2021towards} & 0.029 & 0.073 & 0.099 & 0.168 & 0.244 & 0.036 & 0.108 & 0.056 & 0.031 & 0.095 & \textbf{0.108} & \textbf{0.151} & 0.236 & 0.038 & 0.110 & 0.059 \\
\midrule
    {\bf Ours} & \textbf{0.013} & \textbf{0.049} & \textbf{0.080} & \textbf{0.134} & \textbf{0.139} & \textbf{0.022} & \textbf{0.074} & \textbf{0.035} & \textbf{0.020} & \textbf{0.073} & 0.110 & 0.193 & \textbf{0.132} & \textbf{0.023} & \textbf{0.092} & \textbf{0.045} \\
\bottomrule
\end{tabular}
}
\vspace{-0.3cm}
\caption{Evaluation of semantic part completion on Scan2CAD~\cite{avetisyan2019scan2cad} in comparison to state-of-the-art part segmentation \cite{jiang2020pointgroup,mo2019structurenet} and semantic part completion \cite{bokhovkin2021towards}.
Our optimizable part priors produce more accurate part decompositions.
}
\vspace{-0.4cm}
\label{tab:part_cmpl_comparison}
\end{table*}

\begin{table*}[bp]
\centering
\resizebox{\textwidth}{!}{
\vspace{-0.5cm}
\begin{tabular}{l|cccccc|cc||cccccc|cc}
& \multicolumn{8}{c||}{Chamfer Distance ($\downarrow$)} & \multicolumn{8}{c}{IoU ($\uparrow$)}\\
\toprule
    Method & chair & table & cab. & bkshlf & bed & bin & class avg & inst avg & chair & table & cab. & bkshlf & bed & bin & class avg & inst avg \\
\midrule
    SG-NN\cite{dai2020sgnn} + MLCVNet\cite{xie2020mlcvnet} + PointGroup\cite{jiang2020pointgroup} & 0.056 & 0.121 & 0.110 & 0.161 & 0.406 & 0.034 & 0.148 & 0.088 & 0.257 & 0.390 & \textbf{0.300} & 0.229 & 0.306 & \textbf{0.488} & 0.328 & 0.293 \\
    MLCVNet\cite{xie2020mlcvnet} + StructureNet\cite{mo2019structurenet} & 0.025 & 0.101 & 0.092 & \textbf{0.090} & 0.359 & 0.041 & 0.118 & 0.059 & 0.480 & 0.356 & 0.195 & 0.331 & 0.267 & 0.342 & 0.329 & 0.413 \\
    Bokhovkin et al.\cite{bokhovkin2021towards} & 0.027 & 0.059 & 0.095 & 0.102 & 0.207 & 0.031 & 0.087 & 0.049 & \textbf{0.548} & \textbf{0.542} & 0.224 & 0.328 & 0.442 & 0.375 & 0.409 & \textbf{0.490} \\
\midrule
    {\bf Ours} & \textbf{0.021} & \textbf{0.051} & \textbf{0.076} & 0.094 & \textbf{0.141} & \textbf{0.025} & \textbf{0.068} & \textbf{0.038} & 0.489 & \textbf{0.542} & 0.272 & \textbf{0.386} & \textbf{0.476} & 0.340 & \textbf{0.416} & 0.461 \\
\bottomrule
\end{tabular}
}
\vspace{-0.3cm}
\caption{Evaluation of part segmentation on Scan2CAD~\cite{avetisyan2019scan2cad}. We evaluate part segmentation only on observed scan geometry, in comparison with state-of-the-art part segmentation \cite{jiang2020pointgroup,mo2019structurenet} and semantic part completion \cite{bokhovkin2021towards}. }
\label{tab:part_seg_comparison}
\end{table*}


\section{Results}
\label{sec:results}


% Close-ups
\begin{figure*}
\begin{center}
    \centering
    \includegraphics[width=0.85\textwidth]{fig/comparison.jpg}
    \vspace{-0.2cm}
    \caption{Qualitative comparison of \OURS{} with point \cite{jiang2020pointgroup,mo2019structurenet} and voxel-based \cite{bokhovkin2021towards} state of the art on ScanNet scans with Scan2CAD+PartNet ground truth. Our joint optimization across part priors enables more consistent, accurate part decompositions.}
    \label{fig:comparisons}
\end{center}%
\end{figure*}

We evaluate our \OURSFULL{} for semantic part completion on real-world RGB-D scans from ScanNet~\cite{dai2017scannet}.
We use the official train/val/test split of 1045/156/ 312 scans.
In order to evaluate part segmentation in these real-world scenes, we use the Scan2CAD~\cite{avetisyan2019scan2cad} annotations of CAD model alignments from ShapeNet~\cite{shapenet2015} to these scenes, and the PartNet~\cite{mo2019partnet} part annotations for the ShapeNet objects.
To construct our part latent space, we train on PartNet and train a projection from train ScanNet objects to their PartNet annotations; we also train all baselines on the same ScanNet+PartNet data.
We consider 6 major object class categories representing the majority of parts, comprising a total of 28 part types.
All methods are provided the same MLCVNet bounding boxes, which contain at least $40\%$ of the closest annotated shape from Scan2CAD\cite{avetisyan2019scan2cad} dataset.

\paragraph{Evaluation Metrics}
Since PartNet shapes aligned to real-world ScanNet geometry do not have precise geometric alignments, due to inexact synthetic-real associations, our evaluation metrics aim to characterize the quality of part decompositions that fit well to the real-world geometry, as well as accurately represent complete object geometry.
We evaluate \emph{accuracy} of the part segmentation with respect to the ScanNet object, and object \emph{completion} with respect to the complete object geometry from PartNet.

\emph{Accuracy} measures part segmentation predictions with respect to PartNet labels projected onto ScanNet object geometry, as a single-sided chamfer distance from the partial ScanNet object to the predicted part decomposition (as we lack complete real-world geometry available for evaluation in the other direction).
\emph{Completion} evaluates a bi-directional Chamfer distance between the predicted part decomposition against the PartNet labeled shape.

For evaluation, we sample $10,000$ points per part from predicted and ground-truth mesh surfaces and transform them to the ScanNet coordinate space.
% We consider all evaluation metrics across each part category corresponding to an object class, and evaluate class average over the categories, and instance average over all shapes. 
Each shape instance is evaluated over a union of predicted and ground-truth parts and then summed to represent shape evaluation. All shape evaluations are averaged to form instance average and the mean of shape category averages results in class average.
% If any predicted or ground-truth part does not correspond to the other, we use the center of the respective shape for evaluation.

To evaluate part segmentation of only the observed input geometry without considering completion, we use Chamfer distance and IoU. 
We project part labels from aligned PartNet shapes and predicted mesh parts onto the ScanNet mesh surface to obtain ground truth and predicted part segmentations. 
% Predicted mesh part labels are projected to ScanNet to obtain predicted part segmentation.
% We similarly use $10,000$ sampled points per part for these metrics.
For further details, we refer to the supplemental.

\vspace{-0.3cm}
\begin{table*}[bp]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cccccc|cc||cccccc|cc}
& \multicolumn{8}{c||}{Chamfer Distance ($\downarrow$) -- Accuracy} & \multicolumn{8}{c}{Chamfer Distance ($\downarrow$) -- Completion}\\
\toprule
    Method & chair & table & cab. & bkshlf & bed & bin & class avg & inst avg & chair & table & cab. & bkshlf & bed & bin & class avg & inst avg \\
\midrule
    w/o Projection Map. & 0.032 & 0.156 & 0.140 & 0.249 & 0.352 & 0.029 & 0.160 & 0.081 & 0.026 & 0.144 & 0.137 & 0.192 & 0.309 & 0.025 & 0.139 & 0.070 \\
    w/o Synthetic Pretrain & 0.026 & 0.079 & 0.116 & 0.158 & 0.152 & 0.035 & 0.094 & 0.052 & 0.029 & 0.097 & 0.132 & 0.206 & 0.234 & 0.033 & 0.122 & 0.061 \\
    w/o Test-Time Opt. & 0.019 & 0.060 & 0.105 & 0.145 & 0.200 & \underline{0.023} & 0.093 & 0.047 & \underline{0.022} & 0.085 & 0.127 & \underline{0.183} & 0.198 & \underline{0.024} & 0.107 & 0.052 \\
    w/o Full-shape Constr. & \underline{0.016} & 0.051 & 0.090 & 0.151 & 0.168 & 0.025 & 0.083 & 0.040 & 0.023 & 0.075 & 0.121 & 0.202 & 0.157 & 0.026 & 0.101 & \underline{0.050} \\
    w/o Segmentation & \textbf{0.013} & \textbf{0.046} & \textbf{0.065} & \textbf{0.120} & \textbf{0.062} & \underline{0.023} & \textbf{0.058} & \textbf{0.030} & 0.035 & 0.084 & 0.118 & 0.195 & 0.203 & 0.034 & 0.112 & 0.061 \\
    w/o Scene Consistency & \underline{0.016} & 0.053 & \underline{0.080} & 0.139 & 0.152 & \underline{0.023} & 0.077 & 0.038 & \textbf{0.020} & \underline{0.074} & \textbf{0.108} & \textbf{0.180} & \underline{0.150} & 0.025 & \underline{0.093} & \textbf{0.045} \\
    {\bf Ours} & \textbf{0.013} & \underline{0.049} & \underline{0.080} & \underline{0.134} & \underline{0.139} & \textbf{0.022} & \underline{0.074} & \underline{0.035} & \textbf{0.020} & \textbf{0.073} & \underline{0.110} & 0.193 & \textbf{0.132} & \textbf{0.023} & \textbf{0.092} & \textbf{0.045} \\
\bottomrule
\end{tabular}
}
\vspace{-0.3cm}
\caption{Ablation study evaluating semantic part completion on Scan2CAD~\cite{avetisyan2019scan2cad}. 
We show the effect of our projection mapping initialization, and test-time optimization to fit to the for our design decisions.
Overall, using both results in the best performance in RGB-D scan part decompositions.
In bold -- the best result, underlined -- the second best result.}
\label{tab:ablations}
\end{table*}


\paragraph{Comparison to state of the art}
Tab.~\ref{tab:part_cmpl_comparison} shows a comparison to state of the art on semantic part completion for real-world ScanNet scans, with qualitative results shown in Fig.~\ref{fig:comparisons}.
We compare with Bokhovkin et al.~\cite{bokhovkin2021towards}, which leverages coarse $32^3$ pre-computed geometric priors for semantic part completion, the state-of-the-art part segmentation approaches StructureNet~\cite{mo2019structurenet} and PointGroup~\cite{jiang2020pointgroup}.
Each of these methods uses the same object detection results from MLCVNet~\cite{xie2020mlcvnet}; since PointGroup does not predict any geometric completion, we provide additional scan completion from SG-NN~\cite{dai2020sgnn}.
For Bokhovkin et al.~\cite{bokhovkin2021towards} we apply Marching Cubes to voxels to extract a surface with which to evaluate.
In contrast to these approaches which estimate part decompositions directly and independently, our \OURS{} enable joint optimization over parts to fit precisely to the observed scan geometry, resulting in improved accuracy and completion performance.
Additional qualitative results are shown in the supplemental.

\paragraph{Part segmentation on 3D scans}
We also evaluate part segmentation in Tab.~\ref{tab:part_seg_comparison}, which considers segmentation of only the observed scan geometry, without any geometric completion.
We intersect each method's part predictions with the original scan geometry to evaluate this part segmentation, in comparison with Bokhovkin et al.~\cite{bokhovkin2021towards}, StructureNet~\cite{mo2019structurenet}, and PointGroup~\cite{jiang2020pointgroup}.
By jointly optimizing over the parts of an object to fit to its observed scan geometry, our approach improves notably in part segmentation performance.


%\paragraph{Ablations}
\smallskip
\noindent \textbf{What is the effect of scene-consistent optimization?}
Tab.~\ref{tab:ablations} and Fig.~\ref{fig:comparisons} show the effect of scene-consistent optimization. 
This improves results over \emph{w/o Scene Consistency}, with a stronger effect on categories that more often have repeated instances (e.g., chair, table, bed in offices, classrooms, hotel rooms).
This more holistic optimization enables more consistent reasoning about objects and their parts in a scene.

% General scenes
% \begin{figure*}
% \begin{center}
%     \centering
%     \includegraphics[width=0.95\textwidth]{fig/add_results.jpg}
%     \vspace{-0.3cm}
%     \caption{Additional qualitative results on ScanNet\cite{dai2017scannet} with Scan2CAD\cite{avetisyan2019scan2cad} and PartNet\cite{mo2019partnet} targets, showing our consistent, complete part decompositions.}
%     \label{fig:scenes}
%     \vspace{-0.9cm}
% \end{center}%
% \end{figure*}

\smallskip
\noindent \textbf{What is the impact of test-time optimization and projection initialization?}
We consider our approach without using a learned projection mapping to the latent part space as initialization for test-time optimization to fit the observed scan geometry and also evaluate only the projection mapping without test-time optimization, shown in Tab.~\ref{tab:ablations}.
The initial projection helps significantly to obtain a good initialization for test-time optimization (\emph{w/o Projection Map}), while the projection results provide a good estimate but imprecise fit to the observed scene geometry (\emph{w/o Test-Time Opt}). 
% By leveraging TTO and projection initialization, we can achieve the best representation of the input scan as its part decomposition.

\smallskip
\noindent \textbf{What is the effect of segmentation and full-shape constraints?}
The effects of full-shape constraints (\emph{w/o Full-shape Constr.}) and dense segmentation (\emph{w/o Segmentation}) are evaluated in Tab.~\ref{tab:ablations}. The full-shape constraint helps to maintain the global shape consistency of the optimized parts during TTO. Dense segmentation guides the TTO optimization constraints (e.g., avoids fitting to clutter; prevents self-intersections between optimized reconstructed parts).


% that one is less important - can move to supp
% \smallskip
% \noindent \textbf{Effect of synthetic pre-training.} 
% We evaluate the effect of synthetic pre-training of the part segmentation and projection mappings to the part and shape latent spaces in Tab.~\ref{tab:ablations} (\emph{w/o Synthetic Pretrain}).
% The additional quantity and diversity of data helps to avoid overfitting to more limited real data.



\paragraph{Limitations}
While our \OURS{} shows strong promise towards accurate, high resolution characterization of semantic parts in real-world scenes required for finer-grained semantic scene understanding, various limitations remain.
Our part latent space is trained in its canonically oriented space, and while we can optimize for shape orientations with ICP, a joint optimization or an equivariant formulation can potentially resolve sensitivity to misaligned orientations.
Finally, our scene-consistent optimization for similar shapes in a scene makes an important step towards holistic scene reasoning, but does not consider higher-level, stylistic similarity that is often shared across objects in the same scene (e.g., matching furniture set for desk, shelves, chair) which could provide notable insight towards comprehensive scene understanding.




==> Neural Part Priors CVPR 2023/sec/5_conclusions.tex <==
\section{Conclusion}

We have presented \OURSFULL{}, which introduces learned, optimizable part priors for fitting complete part decompositions to objects detected in real-world RGB-D scans.
We learn a latent part space over all object parts, characterized with learned neural implicit functions.
This allows for traversing over the part space at test time to jointly optimize across all parts of an object such that it fits to the observed scan geometry while maintaining consistency with any similar detected objects in the scan.
This results in improved part segmentation as well as completion in noisy, incomplete real-world RGB-D scans.
We hope that this help to open up further avenues towards holistic part-based reasoning in real-world environments. 
